Decoding Decoders: Finding Optimal Representation Spaces for Unsupervised Similarity Tasks

Experimental evidence indicates that simple models outperform complex deep networks on many unsupervised similarity tasks. We provide a simple yet rigorous explanation for this behaviour by introducing the concept of an optimal representation space, in which semantically close symbols are mapped to representations that are close under a similarity measure induced by the model's objective function. In addition, we present a straightforward procedure that, without any retraining or architectural modifications, allows deep recurrent models to perform equally well (and sometimes better) when compared to shallow models. To validate our analysis, we conduct a set of consistent empirical evaluations and introduce several new sentence embedding models in the process. Even though this work is presented within the context of natural language processing, the insights are readily applicable to other domains that rely on distributed representations for transfer tasks.

==> acronyms/f.tex <==
\newacronym{fs}{FS}{FastSent}
\newacronym{ft}{FT}{Fourier Transform}

==> sections/acknowledgements.tex <==
\subsubsection*{Acknowledgments}

We owe our collective soul to Amazon.


==> sections/related_work.tex <==
\section{Unsupervised Sentence Representations}
\label{sec:related_work}

Based on the success of word-embeddings, many distributed sentence representations are derived from straightforward
functions of constituent word vectors, such as the sum or average \citep{Mitchell2010, Milajevs2014a, Wieting2016, Arora2017}.
 Such models can yield surprisingly high-quality representations, but naturally cannot leverage any contextual information for
 building sentence representations, leading some researchers to move towards more powerful embedding models.

Inspired by the word vector learning procedure by \cite{Mikolov2013a} and the encoder-decoder framework of \cite{Cho2014}, \cite{Kiros2015}
showed that it is possible to learn high-quality generic sentence representations from unlabelled data by leveraging a \emph{sentence-level distributional hypothesis} \citep{Polajnar2015}.
Their model, SkipThought, uses a \gls{rnn} encoder and two \gls{rnn} decoders to predict for any given sentence its two adjacent sentences.

SkipThought has enjoyed impressive results on many supervised transfer benchmarks, particularly when implemented with layer normalisation \citep{Ba2016}.
In these benchmarks, the encoder is fixed after training on a separate unannotated dataset and then used as a feature extractor for a simpler model (such as logistic regression) for the task in question.
In this setting, SkipThought with layer normalisation is currently considered to be one of the best general purpose sentence-level encoders \citep{Conneau2017}, although some recent models have begun to surpass it \citep{Gan2017}.

In contrast, the SkipThought model has proved notably less successful on unsupervised similarity tasks \citep{Hill2016, Conneau2017}.
These benchmarks measure how the cosine distance between sentence pairs correlates with corresponding human judgements of semantic similarity.
Since no additional model is being trained in this scenario, the encoder is evaluated on the merits of its learned representations.
While this shortcoming of SkipThought and \gls{rnn}-based models in general has been pointed out, to the best
of our knowledge, it has never been systematically addressed in the literature before.
Worth noting is the work by \cite{Wieting2017}, which observes a similar discrepancy between the performance of \gls{rnn}s and simply averaging
word vectors, and develops new models based on these insights.  However, their models are trained on a supervised dataset of aligned sentences or paraphrases, as distinct from our unsupervised setting.

\cite{Hill2016} has proposed a conceptually similar approach, FastSent, which replaces SkipThought's computationally expensive
\gls{rnn} encoder and decoders with much simpler \gls{bow} versions.
Interestingly, this change made FastSent among state-of-the-art on unsupervised similarity tasks, but dramatically reduced the performance on
supervised benchmarks \citep{Hill2016, Conneau2017}.
More recent work like \cite{Pagliardini2017} has both improved upon FastSent and begun to close the performance gap with SkipThought in
supervised transfer tasks, but the discrepancy in performance still calls for an explanation.

Others in the literature have recognised the need to analyse the geometric characteristics of representation spaces \citep{Almahairi2015, Schnabel2015}.
Most relevantly, \cite{Hill2016} concluded that
``Deeper, more complex models are preferable for representations to be used in supervised systems,
but shallow log-linear models work best for building representation spaces that can be decoded with simple
spatial distance metrics.''  
The framework presented in \Cref{sec:optimal-representation-space} allows us to extend and refine this statement,
via an analysis of optimal representation spaces for these types of models.

